PAUMER: Patch Pausing Transformer for Semantic Segmentation

We study the problem of improving the efficiency of segmentation transformers by using disparate amounts of computation for different parts of the image. Our method, PAUMER, accomplishes this by pausing computation for patches that are deemed to not need any more computation before the final decoder. We use the entropy of predictions computed from intermediate activations as the pausing criterion, and find this aligns well with semantics of the image. Our method has a unique advantage that a single network trained with the proposed strategy can be effortlessly adapted at inference to various run-time requirements by modulating its pausing parameters. On two standard segmentation datasets, Cityscapes and ADE20K, we show that our method operates with about a $50\%$ higher throughput with an mIoU drop of about $0.65\%$ and $4.6\%$ respectively.

==> results/baseline.tex <==
\begin{table}
    \centering
    \begin{tabularx}{.95\textwidth}{@{}XXXX@{}}
        \toprule
        Method & Backbone & Config & mIoU \\
        RP &  ViT-T & \\
        \bottomrule
    \end{tabularx}
    \caption{Cityscapes}
\end{table}


\begin{table}
    \centering
    \begin{tabularx}{.95\textwidth}{@{}XXXXX@{}}
        \toprule
        Method & Backbone & Config & mIoU & Im/sec\\
        \bottomrule
    \end{tabularx}
    \caption{ADE20K}
\end{table}

==> results/main_table.tex <==
\newcolumntype{A}{>{$}X<{$}}
\definecolor{Azure}{RGB}{0, 127, 255}
\definecolor{grey}{gray}{0.3}
\newcommand{\tra}[1]{\textcolor{Azure}{#1}}
\begin{table}
    \centering
    \begin{minipage}[t]{.4\linewidth}
        {\footnotesize
            \centering
            \begin{tabularx}{.95\textwidth}{@{}>{\color{grey}}lcA@{}}
                \toprule
                Method                                      & Backbone  & \text{mIoU} \% \\\toprule
                FCN\citep{shelhamer2017fully}               & ResNet-50 & 72.64          \\
                BiSeNetV2\citep{yu2021bisenet}              & -         & 73.21          \\
                ANN\citep{zhu2019asymmetric}                & ResNet-50 & 78.88          \\
                DeepLabV3+\citep{deeplabv3plus2018}         & ResNet-50 & 79.83          \\
                \midrule
                \tra{SETR}\citep{zheng2021rethinking}       &           &                \\
                \tra{Segmenter}\citep{strudel2021segmenter} &           &                \\
                \tra{\Paumer-T}                             &           &                \\
                \bottomrule
            \end{tabularx}}
        \caption{Cityscapes}
    \end{minipage}\hfill
    \begin{minipage}[t]{.6\linewidth}
        {\footnotesize
            \centering
            \begin{tabularx}{0.9\textwidth}{@{}lccA@{}}
                \toprule
                Method                              & Backbone                         & Im/sec & \text{mIoU} \\\toprule
                ANN\citep{zhu2019asymmetric}        & ResNet-50                        & 350    & 41.74       \\
                UperNet\citep{xiao2018unified}      & ConvNext-T\citep{liu2022convnet} & 350    & 46.11       \\
                DeepLabV3+\citep{deeplabv3plus2018} & ResNet-50                        & 350    & 43.95       \\
                \bottomrule
            \end{tabularx}}
        \caption{ADE20K}
    \end{minipage}%\vspace{1pt}
    \caption{The cited baselines are based on the models available in the opensource library
        mmsegmentation\citep{mmseg2020}, with similar training budget as our training procedure..}
\end{table}

\input{results/baseline.tex}
